Controlled Occupied Processes and Viscosity Solutions

We consider the optimal control of occupied processes which record all positions of the state process. Dynamic programming yields nonlinear equations on the space of positive measures. We develop the viscosity theory for this infinite dimensional parabolic $occupied$ PDE by proving a comparison result between sub and supersolutions, and thus provide a characterization of the value function as the unique viscosity solution. Toward this proof, an extension of the celebrated Crandall-Ishii-Lions (second order) Lemma to this setting, as well as finite-dimensional approximations, is established. Examples including the occupied heat equation, and pricing PDEs of financial derivatives contingent on the occupation measure are also discussed.

==> Junk.tex <==
\section{Standard Time Occupied Processes}
\label{sec:StdTime}

{\mc{This is what I think is going on.
 In the definition
of $\tilde{\cO}$ we have the  flexibility to use $\d \langle X \rangle_s$ or
any thing like $(...)\d t$.  Here is choose $(...)=1$.}}

{\mc{If this is correct, my problem is this.  In the section
we define the occupational measure.  We say
occupational measure of a process $X$ and use $X$ both in the dirac measure also in 
the quadratic variation.  But when we stop 
using $X$ in the quadratic variation, then the pair
$\cO, X$ is simply a solution to the SDE. }}

{\mc{All of these are fine but we need 
say that at the very beginning when we first define $\sO$.}}

We adapt the above results to controlled processes enlarged by their \textit{standard time occupation flow} \begin{equation}
\label{eq:occFlowStd}
\tilde{\cO} = (\tilde{\cO}_t)_{t\ge 0}, \quad 
\tilde{\cO}_t(B) =
\int_0^t\mathds{1}_B (X_s) 
ds ,  \quad B\in \sB(\R^d).
\end{equation}  %\text{tr}(\d \langle X \rangle_s)
Accordingly, we assume that $(\tilde{\cO}^{\alpha},X^{\alpha})$ is  a strong solution of the occupied stochastic differential equation (OSDE), 
\begin{align}
  d\tilde{\cO}_t^{\alpha} &= \delta_{X_t^{\alpha}} dt, \label{eq:OSDEOccStd}\\[0.5em]
    dX_t^{\alpha} &= b(\tilde{\cO}_t^{\alpha},X_t^{\alpha},\alpha_t)dt + \sigma(\tilde{\cO}_t^{\alpha},X_t^{\alpha},\alpha_t)dW_t.\label{eq:OSDEStd}
\end{align}
Since $|\tilde{\cO}_t^{\alpha}|=t$, the exit time $\tau^\alpha = \inf\{t\ge 0 : (\calO_t^{\alpha},X_t^{\alpha})\notin \sD_{T}\}$ in \eqref{eq:controProblem} equals  $T$ and the stochastic  control problem  translates to
\begin{equation}\label{eq:controProblemStd}
    \text{minimize }  \;  J(\mo,x,\alpha) := \E^{\Q}_{\mo,x}\left[\int_{0}^{T-|\mo|} \ell(\tilde{\cO}_{s}^{\alpha},X_{s}^{\alpha}, \alpha_s) ds  + g(\tilde{\cO}_{T-|\mo|}^{\alpha},X_{T-|\mo|}^{\alpha})\right] \  \text{ over } \  \alpha \in \calA.
\end{equation}
The associated dynamic programming equation is 
\begin{subnumcases}{}
-\partial_{\mo}u + \sH(\mo,x,\nabla u,\nabla^2u) = 0 & \text{ on } \ \ $\sD_{T}$, \label{eq:HJBn12}\\[0.25em] 
      u = g, & \text{ on } \ $\partial \! \sD_{T} $, \label{eq:HJBn22} 
  \end{subnumcases} 
  with the rather classical Hamiltonian 
\begin{equation}\label{eq:HamiltonianStd}
 \sH(\mo,x,\Delta, \Gamma) = -\inf_{a \in A} \Big( 
     b(\mo,x,a) \cdot \Delta + \frac{1}{2}\textnormal{tr}( (\sigma \sigma^{\! \top})(\mo,x,a) \Gamma)  
     + \ell (\mo,x,a) \Big).
\end{equation} 
We suppose that the cost functions $\ell,g$ satisfy  \cref{asm:cost}.  As the flow $\tilde{\cO}$ does not entail the quadratic variation of $X^{\alpha}$, %hence $\lVert \sigma(\mo,x,a) \rVert_{F}^2$, 
we make  slightly different assumptions on the coefficient $\sigma$. 
\begin{assumption}
\label{asm:GrowthLipStd} 
 There exists $c_*\ge 1$  such that for all $(\mo,x), (\mo',x')
\in \sD$, $a \in A$,  
 \begin{align}
         &\lVert \sigma(\mo,x,a) \rVert_{F}  \le c_*
         (1+\rho(\mo,x)), \label{eq:growth}
         \\ &\lVert \sigma(\mo,x,a) - \sigma(\mo',x',a)\rVert_{F} 
         \le c_*\rho(\mo-\mo',x-x'). \label{eq:Lipschitz}
\end{align}
\end{assumption}
% \begin{assumption}
% \label{asm:GrowthLipStd} 
%  There exists $c_*\ge 1$  such that for all $(\mo,x), (\mo',x')
% \in \sD$, $a \in A$,  
%  \begin{align}
%          &|b(\mo,x,a)| + \lVert \sigma(\mo,x,a) \rVert_{F}  \le c_*
%          (1+\rho(\mo,x)), \label{eq:growth}
%          \\ &|b(\mo,x,a)-b(\mo',x',a)| + \lVert \sigma(\mo,x,a) - \sigma(\mo',x',a)\rVert_{F} 
%          \le c_*\rho(\mo-\mo',x-x'). \label{eq:Lipschitz}
% \end{align}
% \end{assumption}
Note also that the ellipticity condition  \eqref{eq:WeakEllipticity} is not needed here since the total mass of $\tilde{\cO}_t^{\alpha}$ is precisely $t$  and in particular does not depend on the diffusion coefficient $\sigma$.

As the dynamic programming equation above is evidently simpler (note that \eqref{eq:HJB12} is  linear in $\partial_{\mo}u$), we state the comparison theorem without proof. 

\begin{theorem}
\label{thm:mainStd}
Suppose that the coefficients $b, \sigma$ satisfy Assumption \ref{asm:GrowthLipStd},
and the cost functions $\ell, g$ satisfy Assumption \ref{asm:cost}. Then, the value function is the unique viscosity solution of
the dynamic programming equation  \eqref{eq:HJBn12}--\eqref{eq:HJBn22}.
\end{theorem} 


\subsection{Quadratic Hedging with Transaction Costs}

\vc{[This is a sketch to wrap my head around it - we can naturally remove this example later. ]}

We adopt a setting similar to \cite{RogersSingh} and refer the interested reader to this article and references therein for further details. 
Let $S = (S_t)_{t\in [0,T]}$ be the price process of a single asset with %risk-neutral 
Black-Scholes dynamics $dS_t = S_t%\sigma(\calO_t,S_t)
\sigma_{\text{\tiny BS}}dW_t$. We are also given an exotic option on $S$  with square-integrable payoff 
$\xi =\varphi(\tilde{\cO}^S_T,S_T), \varphi\in \sC_b(\partial \sD_T),$
where $\tilde{\cO}^S$ is the (standard time) occupation flow of $S$. %We assume that $\xi$ is . 
The seller of the option hedges the contract through the replication strategy
$$Y^{\alpha}_t = \E^{\Q}[\xi] + \int_0^t \Delta_u^{\alpha} dS_u, \quad \Delta_u^{\alpha} = \int_0^{t}\alpha_u du,  $$
such that $Y^{\alpha}_T$ is close to $\xi$  in the $L^2(\Q)$ sense as we shall see  in \eqref{eq:QuadHedging}. %\vc{[or optimize over $Y_0$ too...]}
The control $\alpha_t\in A := \R$ thus characterizes the \textit{trading speed} of the delta-hedge, namely the instantaneous change in the number of shares held at time $t$. %delta-hedging strategy
%X_0 + \int_0^t \Delta_u^{\alpha} S_u\sigma_{\text{\tiny BS}}dW_u
We also assume that any trade incurs  proportional transaction costs $\eta |\alpha_t| S_t$ for some parameter $\eta > 0$; See for instance \cite{RogersSingh}. The seller therefore aims to 
\be \label{eq:QuadHedging}
\text{minimize } \E^{\Q}\left[(\xi - Y^{\alpha}_T)^2 + \int_0^T \eta |\alpha_t|S_t dt\right]  \; \text{  over } \alpha \in \sA.
\ee%\E^{\Q}[\int_0^T \eta |\alpha_t|S_t dt  + (\xi - Y^{\alpha}_T)^2]

Let us rewrite the above problem in the form \eqref{eq:controProblemStd}. %Note that $dY_t = \alpha_t S_t\sigma_{\text{\tiny BS}}dW_t$ 
Introduce  $X^{\alpha} %= (X^{1,\alpha},X^{2,\alpha},X^{3,\alpha}) 
= ( S,\Delta^{\alpha},Y^{\alpha})$ %, hence $d = 3$. 
%We then  easily verify 
and observe that $X^{\alpha}$ together with $\tilde{\cO}^{\alpha} = \int_0^{\cdot} \delta_{X^{\alpha}_u
}du$ solves the controlled OSDE  \eqref{eq:OSDEOccStd}-\eqref{eq:OSDEStd} with (note that $X^{\alpha}$ is driven by a single Brownian motion)
$$b(\mo,x,a)  = \begin{pmatrix} 0 \\ a \\ 0
\end{pmatrix}, \quad  \sigma(\mo,x,a) = \begin{pmatrix}
    x_1\sigma_{\text{\tiny BS}} & 0 &  0\\
    0 & 0 &  0\\
    a x_1 \sigma_{\text{\tiny BS}} & 0 &  0
\end{pmatrix}, \quad  x = (x_1,x_2,x_3), \; a\in \R.$$
Moreover,  $\tilde{\cO}_T^{\alpha}(B \times \R^2) = \int_0^t \mathds{1}_{B}(X_u^{\alpha,1})du = \tilde{\cO}_T^S(B)$ for all $B\in \sB(\R)$,  so we can write $\xi= \varphi(\tilde{\cO}^{\alpha}_T(\cdot\times \R^2),X_T^{\alpha,1})$.  We can finally set $g(\mo,x,a) = (\varphi(\mo(\cdot \times \R^2),x_1) - x_3)^2$ and $\ell(\mo,x,a) = \eta |a| x_1$ in 
\eqref{eq:controProblemStd} to recover the hedging problem \eqref{eq:QuadHedging}. 


\vc{[\textbf{Note:} All assumptions in \cref{thm:mainStd} are satisfied except the boundedness of $\ell,g$. Can we still show that is the unique viscosity solution of \eqref{eq:HJB12UVM}--\eqref{eq:HJB22UVM}? First, the  value function is bounded. Indeed, assuming $t = |\mo| = 0$, then 
$$0\le v_0 \le J(0,(S_0,\Delta_0,Y_0),\alpha \equiv 0 ) = \E^{\Q}[(\xi - Y_0)^2] <\infty \quad \text{(recall that $\xi \in L^2(\Q)$)}.$$
Or change the quadratic cost to $(\xi - Y^{\alpha}_T)^+$ (no penalty if $Y^{\alpha}_T$ superhedges $\xi$) which is bounded because $\varphi$ is bounded. 
}




%========== Appendix B, step 3, OLD VERSION (didn't work) ===========%
Moreover, for each $k\in \N$,
\begin{align*}
    \frac{1}{2}\E^{\Q}[\sup_{t\le T}(\cO_{t}-\cO_t')(f_k)^2] &= (\mo-\mo')(f_k)^2 + T\E^{\Q}[\int_0^T | f_k(X_t)\lambda_t -  f_k(X_t')\lambda_t'|^2dt.
\end{align*}
Next, we use the inequality $|f\lambda - f'\lambda'| \le |f - f'| |\lambda| + |f'||\lambda-\lambda'|$ and Cauchy-Schwarz to obtain 
\begin{align*}
    \frac{1}{2}| f_k(X_t)\lambda_t -  f_k(X_t')\lambda_t'|^2 &\le |f_k(X_t) - f_k(X_t')|^2 |\lambda_t|^2 + |f_k(X_t')|^2|\lambda_t-\lambda_t'|^2 \\[0.5em]
    &\le \lVert \nabla f_k\rVert_{\infty}^2|X_t - X_t'|^2 |\lambda_t|^2 + \lVert f_k\rVert_{\infty}^2|\lambda_t-\lambda_t'|^2 \\[0.5em]
    &\le c_*^2\lVert f_k\rVert_{\sC^1}^2[ (1+\rho(\cO_{t},X_t))^2 + 1]\rho(\cO_{t}-\cO_t',X_{t}-X_t')^2,
\end{align*}
where we apply both the growth and Lipschitz satisfied by $\lambda$ in the last inequality. 
Setting $c_1 := 2Tc_*^2(\E^{\Q}[\sup_{t\le T} (1+\rho(\cO_{t},X_t))^2]+1)$ and recalling that $\sum\nolimits_k\lVert f_k\rVert_{\sC^1}^2\le 1$, we obtain
\begin{align*}
  \frac{1}{2}\E^{\Q}[\sup_{t\le T}\varrho(\cO_{t}-\cO_t')^2] \le \sum\nolimits_k\E^{\Q}[\sup_{t\le T}(\cO_{t}-\cO_t')(f_k)^2] 
  \le \varrho(\mo - \mo')^2 +  c_1  \int_0^TR(t) dt.
     %&\le \varrho(\mo - \mo')^2 + c_*^2T\int_0^T\E^{\Q}[ (1+\rho(\cO_{t},X_t))^2 + \rho(\cO_{t}-\cO_t',X_{t}-X_t')^2]dt.
\end{align*}
Altogether, we obtain
\begin{align*}
    R(T)&\le \E^{\Q}[\sup_{t\le T}\varrho(\cO_{t}-\cO_t')^2] + \E^{\Q}[\sup_{t\le T}|X_{t}-X_t'|^2] 
    \le 3\rho(\mo-\mo',x-x')^2 + c_2\int_0^TR(t) dt
\end{align*}
where $c_2 = 3c_*^2((1+c_1)T + 4)$. We conclude from Grönwall's Lemma that $R(T) \le 3e^{c_2T}\rho(\mo-\mo',x-x')^2$. 
%========== OLD VERSION END ===========%




\section{Proof of \cref{prop:Ito}}%Continuity of the Value Function}
\label{sec:Itoproof}
%======== Proof of Ito formula ======%
\begin{proof} 
  Given $t\ge 0$, let   $0=t_0 < \cdots < t_N = t$ be a sequence of partitions of $[0,t]$ that satisfies    $\max_{n\le N}|t_{n} - t_{n-1}|\to 0$ % \Delta_N:= 
  as $N\to \infty$. Consider  the piecewise constant process 
  \begin{equation}\label{eq:piecewiseconstantX}
      X^{N}_s = \sum_{n} X_{t_{n-1}}\mathds{1}_{[t_{n-1},t_{n})}(s) + X_t\mathds{1}_{\{s = t\}}, \quad  s \le t.
  \end{equation}
  %Write $\phi_t = \phi(\cO^{\alpha}_t,X_t^{\alpha},\alpha_t)$ for $\phi \in \{b,\sigma,\lambda\}$ 
Write also $\Lambda_t = \int_0^t\lambda_sds$ and introduce the discretized occupation flow
        \vc{$\cO^{N}_{s}  := \int_0^s \delta_{X_u^N} d\Lambda_u$}. \vc{[the increments $\Delta_n^{\! \Lambda}$ are introduced later]}
  % \begin{equation}
  %        \cO^{N}_{s} \  \vc{:=} {\color{blue}\int_0^s \delta_{X_u^N} d\Lambda_u = \sum_{t_n \le s} \vc{\delta_{X_{t_{n-1}}}}\Delta_n^{\! \Lambda}}, \quad \Delta_n^{\! \Lambda} = \Lambda_{t_{n}} - \Lambda_{t_{n-1}}. %t_{n+1}-t_n.  %\lambda_{t_n} \Delta t_n, \quad \Delta t_n = t_{n+1}-t_n. 
  % \end{equation}
  %{\color{blue}(This equality is not true!)}
  %Note that $\Delta_n^{\! \Lambda}$ depends on $N$. 
  %Note that $\cO^{N}$ coincides with the occupation flow of the piecewise constant process $$X^{N}_s = \sum_{n\le N} X_{t_n}\mathds{1}_{[t_n,t_{n+1})]}(s) + X_t\mathds{1}_{\{s = t\}}, \quad s \le t.$$ 
  We first establish that $\lim_{N\to \infty}\varrho( \cO_{s} - \cO^{N}_{s}) = 0$ uniformly in  $s\le t$, $\Q-$almost surely.
  For each $k\in \N$ and $f_k$ introduced in \cref{ssec:cylindrical}, we compute 
  \begin{align*}
     &|(\cO_{s} - \cO^N_{s})(f_k)|^2 = \Big|\int_0^s (f_k(X_u) -  f_k(X_u^N))d\Lambda_u\Big|^2  \\[0.5em]
     &\le \Lambda_s\int_0^s | f_k(X_u) -  f_k(X_u^N)|^2d\Lambda_u \le  \Lambda_s  \int_0^s \lVert f_k\rVert_{\sC^1}^2 |X_u -  X_u^N|^2d\Lambda_u.
  \end{align*}
  As the last term  is nondecreasing in $s$ for all $k$, %this leads to the bound  %
  we can  set $s=t$ to obtain 
    \begin{align*}
     \sup_{s\le t} \varrho( \cO_{s} - \cO^{N}_{s})^2 %\sum_{k\in \N}|(\cO_{s} - \cO^N_{s})(f_k)|^2 
     \le  \sum_{k\in \N} \Lambda_t\int_0^t \lVert f_k\rVert_{\sC^1}^2|X_u -  X_u^N|^2d\Lambda_u \le \Lambda_t\int_0^t |X_u -  X_u^N|^2d\Lambda_u.  
  \end{align*}
For $\Q-$almost all $\omega \in \Omega$, $s \mapsto X_s(\omega)$ is uniformly continuous on the compact $[0,t]$, hence it admits a  modulus of continuity $\frakm:\R_+\to\R_+$ (that depends on $\omega$). %We therefore   conclude that  %, i.e.,  $\frakm$ is nondecreasing and satisfies  $\lim_{\Delta \downarrow }\frakm(\Delta) = 0$. 
Consequently,
    \begin{align*}
     \int_0^t |X_u -  X_u^N|^2d\Lambda_u = \sum_{n\le N} \int_{t_{n-1}}^{t_n} |X_u -  X_{t_{n-1}}|^2d\Lambda_u  %= \frakm(\Delta_N)^2 \sum_{n\le N} \int_{t_{n-1}}^{t_n} d\Lambda_u 
     \le  \frakm\! \big(\max_{n\le N}|t_{n} - t_{n-1}|\big)^2 \Lambda_t \to 0, \quad N\to \infty,  %\frakm(\Delta_N)^2 \sum_{n\le N} \int_{t_{n-1}}^{t_n} d\Lambda_u  \frakm(\Delta_N)^2
  \end{align*}
  which shows that $\lim_{N\to \infty}\sup_{s\le t} \varrho( \cO_{s} - \cO^{N}_{s})^2 =0$. 
 Together with the continuity of $v$, we also have   $  v(\calO_{s}^N,X_{s}) \to  v(\calO_{s},X_{s})$ for all $s\le t$. 
 Next, we write 
   %  \begin{align}
   %      v(\calO_{t}^N,X_{t}) -  v(\calO_{0}^N,X_{0}) 
   %         &= \sum_{n\le N}  ( v(\calO_{t_{n}}^{N},X_{t_{n}}) -  v(\calO_{t_{n}}^N,X_{t_{n-1}})).\label{eq:dOcc}\\[0.25em] 
   %      &+ \sum_{n\le N}  ( v(\calO_{t_{n}}^N,X_{t_{n-1}}) -  v(\calO_{t_{n-1}}^N,X_{t_{n-1}})).\label{eq:dIto}
   % \end{align}
   \begin{align}
        v(\calO_{t}^N,X_{t}) -  v(\calO_{0}^N,X_{0}) 
           &= \sum_{n\le N}  ( v(\calO_{t_{n}}^{N},X_{t_{n}}) -  v(\calO_{t_{n-1}}^N,X_{t_{n}})).\label{eq:dOcc}\\[0.25em] 
        &+ \sum_{n\le N}  ( v(\calO_{t_{n-1}}^N,X_{t_{n}}) -  v(\calO_{t_{n-1}}^N,X_{t_{n-1}})).\label{eq:dIto}
   \end{align}
   % \begin{align}
   %      v(\calO_{t},X_{t}) -  v(\calO_{0},X_{0}) 
   %      &= \sum_{n\le N} ( v(\calO_{t_{n+1}},X_{t_{n+1}}) -  v(\calO_{t_{n+1}}^{N},X_{t_{n+1}}))\label{eq:do}\\
   %    &+  \sum_{n\le N} ( v(\calO_{t_{n+1}}^N,X_{t_{n+1}}) -  v(\calO_{t_{n}}^{N},X_{t_{n+1}}))\label{eq:do}\\
   %         &+ \sum_{n\le N}  ( v(\calO_{t_{n}}^{N},X_{t_{n+1}}) -  v(\calO_{t_{n}},X_{t_{n+1}})).\label{eq:dx}\\ 
   %      &+ \sum_{n\le N}  ( v(\calO_{t_{n}},X_{t_{n+1}}) -  v(\calO_{t_{n}},X_{t_{n}})).\label{eq:dx}
   % \end{align}
   From the classical It\^o's formula, the weak convergence of $\cO^N_s$ to $\cO_s$ for all $s\le t$, and the continuity of the data, the  sum \eqref{eq:dIto} converges to %\vc{[add details if needed]}
   $$\int_0^t\Big(b_s \cdot \nabla v+  \frac{1}{2}\textnormal{tr}(\sigma_s \sigma_s^{\! \top} \nabla^2 v) \Big)(\calO_s,X_s) ds + \int_0^t \nabla  v(\calO_s,X_s)\cdot \sigma_s dW_s.$$
   It remains to show that \eqref{eq:dOcc} converges to $\int_0^t \NT_s  \pmo v(\calO_s,X_s) ds. $
   % \begin{equation}
   %     \lim_{N\to \infty} \sum_{n\le N} ( v(\calO_{t_{n+1}},X_{t_{n+1}}) -  v(\calO_{t_{n}}^N,X_{t_{n+1}})) = \int_0^t \NT_s  \pmo v(\calO_s,X_s) ds
   % \end{equation}
   \vc{Define $\Delta_n^{\! \Lambda} = \Lambda_{t_{n}} - \Lambda_{t_{n-1}}$ so that $\cO^{N}_{t_n} = \sum_{m< n} \delta_{X_{t_{m-1}}}\Delta_m^{\! \Lambda}}$, and introduce the function }
   $$\vc{\psi_n(h) =  v(\calO_{t_{n}}^{N} - h\delta_{X_{t_{n-1}}} ,X_{t_{n}}), \quad h\ge 0.}$$ 
\vc{Then 
    $\psi_n(0) =  v(\calO_{t_{n}}^N,X_{t_{n}})$, $\psi_n(\Delta_n^{\! \Lambda}) =  v(\calO_{t_{n-1}}^N,X_{t_{n}})$, we obtain %from the mean value theorem 
using a first order Taylor expansion that  %:} $\psi(1) = \psi(0) + \psi'(0) + r_n$
   % \begin{align*}
   %      v(\calO_{t_{n}}^N,X_{t_{n}}) -  v(\calO_{t_{n-1}}^N,X_{t_{n}}) = \psi_n(0)-\psi_n(\Delta_n^{\! \Lambda})
   %     = \pmo  v(\calO_{t_{n}}^{N},X_{t_{n}})\Delta_n^{\! \Lambda}+ r_n(\Delta_n^{\! \Lambda}),
   % \end{align*}
  \begin{align*}
        v(\calO_{t_{n}}^N,X_{t_{n}}) -  v(\calO_{t_{n-1}}^N,X_{t_{n}}) = \psi_n(0)-\psi_n(\Delta_n^{\! \Lambda})
       = \delta_{\mo}  v(\calO_{t_{n}}^{N},X_{t_{n}})(X_{t_{n-1}})\Delta_n^{\! \Lambda}+ r_n(\Delta_n^{\! \Lambda}),
   \end{align*}}
 \vc{where $r_n(\cdot)$ satisfies %$|r_n(\Delta)| \le c_n \Delta$ for some constant $c_n$.  %
 $\lim_{\Delta \downarrow 0}\frac{r_n(\Delta)}{\Delta} = 0$. 
   In terms of the discretized process $X^N$ in \eqref{eq:piecewiseconstantX}, we can thus write 
      \begin{align*}
        \sum_{n\le N}  ( v(\calO_{t_{n}}^{N},X_{t_{n}}) -  v(\calO_{t_{n-1}}^N,X_{t_{n}})) &=%\int_0^t \pmo  v(\calO_{s}^{N},X_{s}^N)d\Lambda_{s}
        \sum_{n\le N}\delta_{\mo}  v(\calO_{t_{n}}^{N},X_{t_{n}})(X_{t_{n-1}})\Delta_n^{\! \Lambda}
        + \sum_{n\le N} r_n(\Delta_n^{\! \Lambda}). 
   \end{align*}
   % \begin{align*}
   %      \sum_{n\le N}  ( v(\calO_{t_{n}}^{N},X_{t_{n}}) -  v(\calO_{t_{n-1}}^N,X_{t_{n}})) &= \int_0^1\int_0^t \pmo  v(\calO_{t_{n-1}}^{N} + h\delta_{X_{s}^N}\Delta_n^{\! \Lambda},X_{s}^N)d\Lambda_{s} dh. 
   % \end{align*}
   Since $\Lambda$ has finite variation (being absolutely continuous), it is easily seen that $\sum_{n\le N} r_n(\Delta_n^{\! \Lambda})\to 0$ as $N\to \infty$.  %it has zero quadratic variation. Hence,  
   %$$\sum_{n\le N} |r_n(\Delta_n^{\! \Lambda})| \le  \sum_{n\le N} c_n (\Delta_n^{\! \Lambda})^2 \le  \sup_{n\le N}c_n \sum_{n\le N} (\Delta_n^{\! \Lambda}^2) \to 0. $$
   %$$\sum_{n\le N} r_n(\Delta_n^{\! \Lambda}) \le C \sum_{n\le N} (\Delta_n^{\! \Lambda})^2 \le C \sup_{n\le N}|\Delta_n^{\! \Lambda}| \sum_{n\le N} \Delta_n^{\! \Lambda} \to 0. $$
We finally conclude %from the continuity of $\pmo  v$  
that 
   $$%\int_0^t \pmo  v(\calO_{s}^{N},X_{s}^N)d\Lambda_{s}
    \sum_{n\le N}\delta_{\mo}  v(\calO_{t_{n}}^{N},X_{t_{n}})(X_{t_{n-1}})\Delta_n^{\! \Lambda} \to \int_0^t   \pmo v(\calO_s,X_s) d\Lambda_s =  \int_0^t \NT_s  \pmo v(\calO_s,X_s) ds.$$
   The proof is complete. }

 %============ OLD CONCLUSION ============%
%    For each $n\le N$, define
%    $$\psi_n(h) = \varphi(\calO_{t_{n-1}}^{N} + h\delta_{X_{t_{n}}} \Delta\Lambda_{t_{n}},X_{t_{n}}), \quad h\in [0,1].$$ 
%    Noting that $\psi_n(0) = \varphi(\calO_{t_{n}}^N,X_{t_{n-1}})$, $\psi_n(1) = \varphi(\calO_{t_{n}}^N,X_{t_{n}})$, we obtain %from the mean value theorem 
% from a first order Taylor expansion that  %:} $\psi(1) = \psi(0) + \psi'(0) + r_n$
%    \begin{align*}
%        \varphi(\calO_{t_{n}}^N,X_{t_{n}}) - \varphi(\calO_{t_{n}}^N,X_{t_{n-1}}) = \psi_n(1)-\psi_n(0) =  \psi_n'(0) + r_n = \pmo \varphi(\calO_{t_{n-1}}^{N},X_{t_{n}})\Delta\Lambda_{t_{n}}+ r_n. 
%        %=\pmo \varphi(\calO_{t_{n-1}}^{N} + h_n\delta_{X_{t_n}}\Delta\Lambda_{t_{n}},X_{t_{n}})\Delta\Lambda_{t_{n}}, 
%    \end{align*}
%    % \begin{align*}
%    %     \varphi(\calO_{t_{n}}^N,X_{t_{n}}) - \varphi(\calO_{t_{n}}^N,X_{t_{n-1}}) =  \int_0^1 d\psi(h) = \int_0^1\pmo \varphi(\calO_{t_{n-1}}^{N} + h\delta_{X_{t_n}}\Delta\Lambda_{t_{n}},X_{t_{n}})\Delta\Lambda_{t_{n}}dh. 
%    %     %=\pmo \varphi(\calO_{t_{n-1}}^{N} + h_n\delta_{X_{t_n}}\Delta\Lambda_{t_{n}},X_{t_{n}})\Delta\Lambda_{t_{n}}, 
%    % \end{align*}
%    %$$\varphi(\calO_{t_{n}}^N,X_{t_{n}}) - \varphi(\calO_{t_{n}}^N,X_{t_{n-1}}) = %\psi(1)-\psi(0) = \psi'(h_n) 
%    %\int_0^1 \psi'(h)dh = \pmo \varphi(\calO_{t_{n-1}}^{N} + h_n\delta_{X_{t_n}}\Delta\Lambda_{t_{n}},X_{t_{n}})\Delta\Lambda_{t_{n}}, $$
%    %for some $h_n\in [0,1]$. Summing the above expression over $n$ and letting  $N$ tend to $\infty$ yields  
%    In terms of the discretized process $X^N$ in \eqref{eq:piecewiseconstantX}, we can write 
%       \begin{align*}
%         \sum_{n\le N}  (\varphi(\calO_{t_{n}}^{N},X_{t_{n}}) - \varphi(\calO_{t_{n-1}}^N,X_{t_{n}})) &=\int_0^t \pmo \varphi(\calO_{s}^{N},X_{s}^N)d\Lambda_{s} + \sum_{n\le N} r_n. 
%    \end{align*}
%    % \begin{align*}
%    %      \sum_{n\le N}  (\varphi(\calO_{t_{n}}^{N},X_{t_{n}}) - \varphi(\calO_{t_{n-1}}^N,X_{t_{n}})) &= \int_0^1\int_0^t \pmo \varphi(\calO_{t_{n-1}}^{N} + h\delta_{X_{s}^N}\Delta\Lambda_{t_{n}},X_{s}^N)d\Lambda_{s} dh. 
%    % \end{align*}
%    For each $h\in [0,1]$, the dominated convergence theorem finally  implies that 
%    $$\int_0^t \pmo \varphi(\calO_{t_{n-1}}^{N} + h\delta_{X_{s}^N}\Delta\Lambda_{t_{n}},X_{s}^N)d\Lambda_{s} \to \int_0^t   \pmo\varphi(\calO_s,X_s) d\Lambda_s =  \int_0^t \NT_s  \pmo\varphi(\calO_s,X_s) ds.$$
%    The proof is now complete. 
%    %$$ \sum_{n\le N}  (\varphi(\calO_{t_{n}}^{N},X_{t_{n}}) - \varphi(\calO_{t_{n-1}}^N,X_{t_{n}})) \longrightarrow  \int_0^t   \pmo\varphi(\calO_s,X_s) d\Lambda_s = \int_0^t \NT_s  \pmo\varphi(\calO_s,X_s) ds.$$
%============ OLD CONCLSION END =========%
\end{proof}



\section*{Proof of \cref{prop:Lipschitz} \vc{(OLD)}}


% \begin{lemma}\label{lem:LipschitzX}
%     \mc{Under the Assumption \ref{asm:standing}, there exists $\hat{c} \in (0,\infty)$ depending only on on $c_*$ and $T$ such that }
%     $$
%     \mc{|v(\mo,x) - v(\mo',x')| \le \hat{c} \ (|x-x'|+ \varrho(\mo-\mo')), 
%     \qquad \forall \mo,\mo' \in \sM_T, \; x\in \R^d.}
%     $$
% \end{lemma}
%\vc{ [ @ Mete:  we actually don't need to separate $x$ and $\mo$, the lemma was not really helpful and I was about to remove it]}
\begin{proof} 
      We  show that $J(\mo,x,\alpha)$ is Lipschitz continuous   with constant $\hat{c}$ (to be determined) \mc{independent} of $\alpha \in \sA$ and $\mo\in \sM_T$. It is then immediate to see that  $v(\mo,x)$ is  Lipschitz continuous  with the same constant.  
    Fix $(\mo,x),(\mo',x') \in \sD_T$, $\alpha \in \sA$, and write $(\cO,X)$, $(\cO',X')$ for  the solution of \eqref{eq:OSDEOcc}-\eqref{eq:OSDE} controlled by $\alpha$ with  initial value $(\mo,x),(\mo',x')$, respectively. Also, the exit times of $(\cO,X)$, $(\cO',X')$ from $\sD_T$ are  denoted by $\tau,\tau'$. 
    First, the triangle inequality gives  
\begin{align*}
   |J(\mo,x,\alpha)  - J(\mo,x',\alpha)| 
   &\le \E^{\Q}[|\int_0^{\tau}\ell(\cO_{s},X_{s},\alpha_s)ds - \int_0^{\tau'}\ell(\cO_{s}',X_{s}',\alpha_s)ds|] \\[1em]
   &+ \E^{\Q}[|g(\cO_{\tau},X_{\tau}) - g(\cO_{\tau'}',X_{\tau'}')|].
\end{align*}
We estimate the terminal and running cost  terms separately. 

\noindent
\emph{Step 1.} (terminal cost). Using the Lipschitz condition satisfied by $g$, then 
\begin{align*}
 \E^{\Q}[|g(\cO_{\tau},X_{\tau}) - g(\cO_{\tau'}',X_{\tau'}')|]
   \le c_* \E^{\Q}[\rho(\cO_{\tau}-\cO_{\tau'}',X_{\tau}-X_{\tau'}')],
\end{align*}
with the parabolic norm $\rho(\mo,x) = \sqrt{\varrho(\mo)^2 + |x|^2}$.  Next, consider  the decomposition, 
\begin{equation}
    \rho(\cO_{\tau}-\cO_{\tau'}',X_{\tau}-X_{\tau'}') \le \rho(\cO_{\tau}-\cO_{\tau'},X_{\tau}-X_{\tau'}) + \rho(\cO_{\tau'}-\cO_{\tau'}',X_{\tau'}-X_{\tau'}').
\end{equation}
We first estimate the second term on the right-hand side of \eqref{eq:appBDecomp}. 

\noindent
\emph{Step 1.a.} (Gr\"onwall's Lemma).
Recalling that  condition \eqref{eq:WeakEllipticity}  implies  $\tau' \le c_*T =: T_*$, we have
\begin{equation}
    \E^{\Q}[\rho(\cO_{\tau'}-\cO_{\tau'}',X_{\tau'}-X_{\tau'}')^2] \le R(T_*), \quad R(t) := \E^{\Q}[\sup_{s\le t\wedge \tau'}\rho(\cO_{s}-\cO_s',X_s-X_s')^2]. %\E^{\Q}[\sup_{s\le c_* T\wedge \tau }\rho(\cO_{s}-\cO_s',X_s-X_s')^2],
\end{equation}
We now derive a bound for  $R(\cdot)$ using Gr\"onwall's Lemma. 
%so it remains to estimate the right-hand side in \eqref{eq:appBBound}. 
%Define  $R(t) = \E^{\Q}[\sup_{s\le t\wedge \tau}\rho(\cO_{s}-\cO_s',X_s-X_s')^2]$ and 
Fix $t\le T_*$ and  write $\varphi_t = \varphi(\cO_t,X_t,\alpha_t)$, $\varphi_t' = \varphi(\cO_t',X_t',\alpha_t)$ with $\varphi \in \{b,\sigma,\lambda\}$. From 
Cauchy-Schwarz and Doob's inequalities, it is classical that 
\begin{align*}
    \frac{1}{3}\E^{\Q} [ \ \sup_{s\le t\wedge \tau' }|X_s-X_s'|^2 ] &\le  |x-x'|^2 + t\E^{\Q}[\int_0^{t\wedge \tau'} |b_s - b_s'|^2ds] + 4 \E^{\Q}[\int_0^{t\wedge \tau'}|\sigma_s - \sigma_s'|^2ds] \\
    &\le |x-x'|^2 + c_*^2(t+4)\int_0^t\E^{\Q}[\sup_{u\le s\wedge \tau'} \rho(\cO_{u}-\cO_u',X_u-X_u')^2]ds\\
    &\le |x-x'|^2 + c_*^2(T_*+4)\int_0^tR(s)ds.
\end{align*}
Moreover, for each $k\in \N$, the triangle inequality and occupation time formula  yields 
\begin{align}
    \sup_{s\le t\wedge \tau'}|(\cO_{s}-\cO_s')(f_k)| &\le |(\mo-\mo')(f_k)| + \int_0^{t\wedge \tau'} | f_k(X_s)\lambda_s -  f_k(X_s')\lambda_s'|ds.
\end{align}
Next,  use $|f\lambda - f'\lambda'| \le |f||\lambda-\lambda'| + |f - f'| |\lambda'|$ and Cauchy-Schwarz inequality  to obtain 
\begin{align}
  | f_k(X_s)\lambda_s -  f_k(X_s')\lambda_s'| &\le |f_k(X_s)||\lambda_s-\lambda_s'|  + |f_k(X_s) - f_k(X_s')| \lambda_s'  \nonumber\\[0.5em]
    &\le \lVert f_k\rVert_{\infty}|\lambda_s-\lambda_s'| + \lVert \nabla f_k\rVert_{\infty}|X_s - X_s'| \lambda_s'   \nonumber\\[0.5em]
    &\le c_*\lVert f_k\rVert_{\sC^1} (1+ \lambda_s')\rho(\cO_{s}-\cO_s',X_{s}-X_s'),
\end{align}
% Next,  use $|f\lambda - f'\lambda'| \le |f - f'| |\lambda| + |f'||\lambda-\lambda'|$ and Cauchy-Schwarz inequality  to obtain 
% \begin{align}
%   | f_k(X_s)\lambda_s -  f_k(X_s')\lambda_s'| &\le |f_k(X_s) - f_k(X_s')| \lambda_s + |f_k(X_s')||\lambda_s-\lambda_s'| \nonumber\\[0.5em]
%     &\le \lVert \nabla f_k\rVert_{\infty}|X_s - X_s'| \lambda_s + \lVert f_k\rVert_{\infty}|\lambda_s-\lambda_s'| \nonumber\\[0.5em]
%     &\le c_*\lVert f_k\rVert_{\sC^1} (\lambda_s  + 1)\rho(\cO_{s}-\cO_s',X_{s}-X_s'),\label{eq:appBintegrand}
% \end{align}
using the Lipschitz property of $\lambda$ in the last inequality. 
Note also that $\int_0^{t\wedge \tau'}\lambda_s' ds \le  \Lambda_\tau' = |\cO_\tau'| = T$. Together with  $\tau'\le T_*$ and  \eqref{eq:appBvarrho}, we obtain by integrating \eqref{eq:appBintegrand} that 
$$ \frac{1}{2}\sup_{s\le t\wedge \tau'}|(\cO_{s}-\cO_s')(f_k)|^2 \le |(\mo-\mo')(f_k)|^2 + c_*^2\lVert f_k\rVert_{\sC^1}^2 (T_*  + T)^2\int_0^t\sup_{u\le s\wedge \tau'} \rho(\cO_{u}-\cO_u',X_u-X_u')^2ds.$$
Using  $\sum\nolimits_k\lVert f_k\rVert_{\sC^1}^2\le 1$, we obtain  by summing over $k$ that 
\begin{align*}
  \frac{1}{2}\E^{\Q}[\sup_{s\le t\wedge \tau'}\varrho(\cO_{s}-\cO_s')^2] %\le \sum\nolimits_k\E^{\Q}[\sup_{s\le t\wedge \tau'}|(\cO_{s}-\cO_s')(f_k)|^2] 
  \le \varrho(\mo - \mo')^2 +   c_*^2 (T  + T_*)^2  \int_0^t R(s) ds.
\end{align*}
Altogether, we have established  that 
\begin{align*}
    R(t)&\le \E^{\Q}[\sup_{s\le t\wedge \tau'}\varrho(\cO_{s}-\cO_s')^2] + \E^{\Q}[\sup_{s\le t\wedge \tau'}|X_{s}-X_s'|^2] 
    \le 3\rho(\mo-\mo',x-x')^2 + C\int_0^{t} R(s) ds
\end{align*}
where $C = c_*^2[3(T+4) + 2(T+T_*)^2]$. We therefore conclude from Grönwall's Lemma that 
$$ \E^{\Q}[\rho(\cO_{\tau'}-\cO_{\tau'}',X_{\tau'}-X_{\tau'}')^2] \le R(T_*) \le 3e^{C  T_*}\rho(\mo-\mo',x-x')^2.$$ 
\emph{Step 1.b.} (exit times). 
We now  treat the remaining term
$$\E^{\Q}[\rho(\cO_{\tau}'-\cO_{\tau'}',X_{\tau}'-X_{\tau'}')^2] = \E^{\Q}[\varrho(\cO_{\tau}'-\cO_{\tau'}')^2]+ \vc{\E^{\Q}[|X_{\tau}'-X_{\tau'}'|^2]}. $$
 Assume that $\tau' \le \tau$.  Using the linear growth of $\lambda$,  observe that for all $k\ge 1$, 
\begin{align*}
    \frac{1}{2}|(\cO_{\tau}-\cO_{\tau'})(f_k)|^2 &= |(\mo-\mo')(f_k)|^2 +  \big(\int_{\tau'}^{\tau} | f_k(X_s)|\lambda_sds \big)^2 \\
    &\le |(\mo-\mo')(f_k)|^2 + c_*^2 \lVert f_k\rVert_{\sC^1}^2  |\tau-\tau'|^2 \sup_{t\le T_*}(1+\rho(\cO_t,X_t))^2.
\end{align*}
Summing over $k$, we obtain
\begin{equation}\label{eq:boundVARRHO}
    \E^{\Q}[\varrho(\cO_{\tau}'-\cO_{\tau'}')^2] \le 2\varrho(\mo-\mo')^2 + 2C^2 \rVert\tau-\tau'\rVert_{L^2(\Q)}^2,
\end{equation}
with the finite constant $C = c_* \E^{\Q}[\sup_{t\le  T_*}(1+\rho(\cO_{t},X_{t}))^2]^{1/2} $. Similarly, it is easily seen that 
\begin{align*}
    \E^{\Q}[|X_{\tau}'-X_{\tau'}'|] &\le 
\end{align*}
\textbf{comment:} with $\E^{\Q}[|X_{\tau}'-X_{\tau'}'|^{\bm{2}}]$ we get terms of order $4$ and I don't think this could be avoided. 
% \begin{align*}
%      \frac{1}{2}\E^{\Q}[|X_{\tau}-X_{\tau'}|^2] &\le \vc{...} \le const.  C \ \rVert\tau-\tau'\rVert_{L^2(\Q)}^2%\E^{\Q}[\int_0^{t\wedge \tau} |b_s|^2ds] + 4 \E^{\Q}[\int_0^{t\wedge \tau}|\sigma_s - \sigma_s'|^2ds]
% \end{align*}
Next, we prove the following lemma.
\begin{lemma} If $\tau,\tau'$ denotes the exit time of $(\cO,X),(\cO',X')$
    respectively, then\\[0.25em] 
    \begin{equation} 
    %\rVert\tau-\tau'\rVert_{L^2(\Q)} \le c_*\lVert \sup_{t\le T^*}  |(\cO_t - \cO_t')(\R^d)| \rVert_{L^2(\Q)}
    |\tau-\tau'| \le c_*\sup_{t\le T^*}  |(\cO_t - \cO_t')(\R^d)|,  \qquad \Q-a.s.
\end{equation}
\end{lemma}
\begin{proof}
    %Suppose that  $\sup_{t\le T_*} |(\cO_t - \cO_t')(\R^d)| \le \delta$
%$$\sup_{t\le T_*} ||\cO_t| - |\cO_t'|| \le \delta \; \Longrightarrow \; |\tau - \tau'|\le c_*\delta.$$
%Indeed, 
Suppose that $\tau'<\tau$ without loss of generality and let $\delta :=\sup_{t\le T_*} |(\cO_t - \cO_t')(\R^d)|$. Then, using $\cO_{\tau'}'(\R^d) = T$ and  the linearity of $\mo \to  \mo(\R)$, we have 
\begin{align*}
    \cO_{\tau'}(\R^d) &= \cO_{\tau'}'(\R^d) + (\cO_{\tau'} - \cO_{\tau'}')(\R^d) \ge T - \delta.
\end{align*}
Moreover, the nondegeneracy condition \eqref{eq:WeakEllipticity} implies that   $$ \cO_{\tau' + s}(\R^d) = \cO_{\tau'}(\R^d) + \int_{\tau'}^{\tau'+s}\lambda_{u}du \ge T-\delta + s/c_*, \quad \forall s\ge 0.$$
Choosing $s = c_*\delta$ therefore gives $\tau \le \tau'+c_*\delta$ and similarly $\tau' \le \tau+c_*\delta$. 
\end{proof}
Combining the above Lemma with \eqref{eq:boundVARRHO} yields
\begin{equation*}
    \E^{\Q}[\varrho(\cO_{\tau}'-\cO_{\tau'}')^2] \le 2\varrho(\mo-\mo')^2 + 2C^2 c_*^2 \E^{\Q}[\sup_{t\le T^*}  |(\cO_t - \cO_t')(\R^d)|^2].
\end{equation*}
Next,  we observe that for all $t\le T_*$,
\begin{align*}
          |(\cO_t - \cO_t')(\R^d)| \le  |(\mo -\mo')(\R^d)| + \int_0^t|\lambda_s-\lambda_s'|ds. 
\end{align*}
\vc{Recalling that the first element of the separating family $(f_k)_{k\in \N}$ is constant, say $f_0 \equiv c_0$ with $c_0\in (0,1)$, we note that   
$$|(\mo -\mo')(\R^d)|^2  = c_0^{-2}|(\mo -\mo')(f_0)|^2\le c_0^{-2}\varrho(\mo -\mo')^2. \qquad (\star)$$}
Moreover, we have from the Lipschitz continuity that 
\begin{align*}
    \int_0^t|\lambda_s-\lambda_s'|ds \le c_*\int_0^t\rho(\cO_s - \cO_s',X_s - X_s')ds \le T_* \sup_{s\le T_*}\rho(\cO_s - \cO_s',X_s - X_s').
\end{align*}
From Step 1.a, we thus obtain that 
\begin{equation*}
    \E^{\Q}[\sup_{t\le T_*}|(\cO_t - \cO_t')(\R^d)|^2] \le 2 c_0^{-2}\varrho(\mo -\mo')^2 + 6c_*e^{C  T_*}\rho(\mo-\mo',x-x')^2.
\end{equation*}
We finally conclude that 
$\E^{\Q}[\varrho(\cO_{\tau}'-\cO_{\tau'}')^2]\le \tilde{C}\rho(\mo-\mo',x-x')^2$, where $\tilde{C} = 2 +  4C^2c_*^2[c_0^{-2} + 3c_*e^{C  T_*}]$. 


\noindent
\emph{Step 2.} (running cost). Assume  $\tau \le \tau' $ and write 
\begin{align*}
    |\int_0^{\tau}\ell(\cO_{s},X_{s})ds - \int_0^{\tau'}\ell(\cO_{s}',X_{s}')ds| &\le   \int_0^{\tau }|\ell(\cO_{s},X_{s},\alpha_s) - \ell(\cO_{s}',X_{s}',\alpha_s)|ds\\
    &+ \int_{\tau }^{\tau' }|\ell(\overline{\cO}_{s},\overline{X}_{s},\alpha_s)|ds.  
\end{align*}
From the growth and Lipschitz property of $\ell$, we obtain
\begin{align*}
    \int_0^{\tau }|\ell(\cO_{s},X_{s},\alpha_s) - \ell(\cO_{s}',X_{s}',\alpha_s)|ds  &\le c_*\int_0^{\tau}\rho(\cO_{s}-\cO_{s}',X_{s}-X_{s}')ds \\[0.5em] 
    &\le c_*T_* \sup_{s\le  \tau}\rho(\cO_{s}-\cO_{s}',X_{s}-X_{s}'), \\[0.5em]
    \int_{\tau }^{\tau'}|\ell(\cO_{s},X_{s},\alpha_s)|ds &\le c_*  (\tau'- \tau) (1+ \sup_{s\le  T_*}\rho(\cO_{s}',X_{s}')). 
\end{align*}
The case $\tau'<\tau$ follows analogously. 
Taking expectation, we obtain 
\begin{align*}
        \E^{\Q}[|\int_0^{\tau}\ell(\cO_{s},X_{s})ds - \int_0^{\tau'}\ell(\cO_{s}',X_{s}')ds|] &\le c_*T_*  \E^{\Q}[ \sup_{s\le  \tau\wedge \tau'}\rho(\cO_{s}-\cO_{s}',X_{s}-X_{s}')] +  C \lVert \tau - \tau'\rVert_{L^2(\Q)},
\end{align*}
with the finite constant $C = c_* \E^{\Q}[(1+\sup_{s\le  T_*}\rho(\cO_{s},X_{s}) \vee \rho(\cO_{s}',X_{s}'))^2]^{1/2} $. 
\vc{[find bound for $\lVert \tau - \tau'\rVert_{L^2(\Q)}$ from  Step 1.b.]}

\end{proof}

